MSL-RAPTOR: A 6DoF Relative Pose Tracker for Onboard Robotic Perception

Determining the relative position and orientation of objects in an environment is a fundamental building block for a wide range of robotics applications. To accomplish this task efficiently in practical settings, a method must be fast, use common sensors, and generalize easily to new objects and environments. We present MSL-RAPTOR, a two-stage algorithm for tracking a rigid body with a monocular camera. The image is first processed by an efficient neural network-based front-end to detect new objects and track 2D bounding boxes between frames. The class label and bounding box is passed to the back-end that updates the object's pose using an unscented Kalman filter (UKF). The measurement posterior is fed back to the 2D tracker to improve robustness. The object's class is identified so a class-specific UKF can be used if custom dynamics and constraints are known. Adapting to track the pose of new classes only requires providing a trained 2D object detector or labeled 2D bounding box data, as well as the approximate size of the objects. The performance of MSL-RAPTOR is first verified on the NOCS-REAL275 dataset, achieving results comparable to RGB-D approaches despite not using depth measurements. When tracking a flying drone from onboard another drone, it outperforms the fastest comparable method in speed by a factor of 3, while giving lower translation and rotation median errors by 66% and 23% respectively.

==> 02_NOT_USED_related_works.tex <==

%
Our method combines and builds upon related work in the areas of object detection, visual tracking, pose estimation, and probabilistic filtering. 
\subsection{Visual data extraction}
%
Our system relies on monocular images as its sensory inputs, and as such we make use of recent advances in computer vision powered by deep learning to extract semantic and geometric information.
Two of the most relevant areas of visual data extraction are detection and tracking. Detection involves identifying an object in an image and locating areas of pixels that represent it. Tracking assumes the object has already been detected in a previous frame and uses that prior to propagate pixels corresponding to projections of the same object in the next frame.

\subsubsection{Detection}
%
YOLOv3~\cite{redmon2018yolov3} and SSD~\cite{wei2016ssd} are two well-known detection methods that take advantage of the fact that object-classification networks are fast by applying this technique at different positions and scales to quickly detect objects. The latest version of YOLO incorporates the ResNet network architecture~\cite{he2016resnet} that is designed to improve training on deep learning networks and has been shown to perform well on image processing tasks. MAVNet~\cite{nguyen2019mavnet} is a network designed specifically for object detection by micro-unmanned aerial vehicles (UAVs), with a focus on fast computation for onboard robotic perception in scenarios that are often more challenging than less-realistic datasets. While previous methods do not make use of the continuity of images in the real-world, some recent works take advantage of sequences of images for detection, for example by using shifting views to differentiate the foreground from the background~\cite{xie2019objectdiscovery}.

\subsubsection{Tracking}
%
Tracking methods leverage the correlation between time and object position for a sequence of images. Given a previous segmentation of an object, an updated region can be found with less computation since it is likely that the object has not moved far between frames. Most of these methods are class agnostic; they can track an object frame-to-frame without knowing anything a priori about the object other than its first location. Siamese networks~\cite{bertinetto2016siamese} have been at the origin of recent state-of-the-art results~\cite{wang2019siammask,li2018siamrpn++}. SiamMask~\cite{wang2019siammask} in particular uses a binary segmentation mask that improves training and provides pixel-wise segmentation and angled bounding boxes of the object. THOR~\cite{sauer2019thor} builds a framework to augment tracking methods by aggregating a set of different templates (i.e. views). 

\subsection{Pose prediction}
%
There are many approaches in the computer vision literature to estimate the pose of an object from a single monocular image, though many require depth-sensing in addition to an RGB image. As this task is more challenging than generating a 2D bounding box, most of these methods do not run in real-time. 

PoseCNN~\cite{xiang2017posecnn} and LieNets~\cite{do2018lienets} use convolutional neural networks (CNN) to regress a pose estimate. A downside of large CNN-based methods is they can be slow, though LieNets is relatively fast at 10 Hz on a desktop GPU. Approaches such as BB8~\cite{rad2017bb8}, SSD-6D~\cite{kehl2017ssd}, DOPE~\cite{tremblay2018dope} and SingleShotPose~\cite{tekin2018ssp} estimate the 2D projections of the 3D bounding box encompassing the object and solve the Perspective-n-Point (PnP) problem to obtain a pose estimate~\cite{lepetit2009epnp}. NOCS~\cite{wang2019normalized} instead presents a category-level canonical representation in which pixel correspondences are found and combined with depth data to estimate the pose.
These methods are the most efficient of the existing deep pose estimation techniques, but even the fastest cannot achieve real-time performance on embedded systems. MSL-RAPTOR is able to achieve these speeds on much more limited hardware by leveraging the relationship between sequential images for speed and memory efficiency.  

\subsection{Pose tracking}
%
For onboard robotic perception it is common to have access to sequences of images. These provide more information that can help pose estimation.
%
Recent works have sought to blend deep learning advances, particularly for perception, with those of probabilistic filtering. PoseRBPF~\cite{deng2019poserbpf} decouples the translation and orientation estimation problems. The translation is estimated and fed into a network that extracts a latent representation of the cropped view of the object. Along with a pre-computed codebook for each object, a Rao-Blackwellized particle filter (PF) is used to estimate orientation. Limiting the PF to just orientation allows this method to reach between 20 Hz for 50 particles to 3 Hz for 400 particles on a desktop GPU. The nature of this filter does not admit knowledge of the object dynamics, which lessens the multi-hypothesis tracking capability offered by a PF. 

6-PACK~\cite{wang20196sixpack} is another pose estimation method that leverages temporal consistency by learning to represent objects by keypoints that are matched between frames. It obtains impressive state-of-the-art category-level pose estimation results, but contrary to MSL-RAPTOR, it relies on RGB-D data and is unable to run real-time on an embedded device.%\todo{Mention energy efficiency?}

The authors of DART~\cite{schmidt2014dart} eschew neural networks and instead perform iterative optimizations given a depth map at each time step and knowing the signed distance function of the tracked object. This method can reach 30 Hz on a powerful GPU, but the assumptions required for sensing and knowledge of the object make it ill-suited to general pose estimation in robotics.

To our knowledge, no method offers MSL-RAPTOR's speed and performance for onboard robot perception.


